Optimizing Distributed Protocols with Query Rewrites [Technical Report]

Distributed protocols such as 2PC and Paxos lie at the core of many systems in the cloud, but standard implementations do not scale. New scalable distributed protocols are developed through careful analysis and rewrites, but this process is ad hoc and error-prone. This paper presents an approach for scaling any distributed protocol by applying rule-driven rewrites, borrowing from query optimization. Distributed protocol rewrites entail a new burden: reasoning about spatiotemporal correctness. We leverage order-insensitivity and data dependency analysis to systematically identify correct coordination-free scaling opportunities. We apply this analysis to create preconditions and mechanisms for coordination-free decoupling and partitioning, two fundamental vertical and horizontal scaling techniques. Manual rule-driven applications of decoupling and partitioning improve the throughput of 2PC by $5\times$ and Paxos by $3\times$, and match state-of-the-art throughput in recent work. These results point the way toward automated optimizers for distributed protocols based on correct-by-construction rewrite rules.

==> x-limitations-future-work.tex <==
\section{Future work}
\label{sec:limitations-future-work}

% In this paper we presented rule-based rewrites to optimize distributed protocols.
% We briefly discuss possible future directions of this work.
% \nc{This is a very long section for future work. While I"m glad you have a lot of ideas, do we really need it?. Most papers only include 3/4 lines, at most}
Query optimization is classically built out of three components: transformation axioms, a cost model, and an algorithm to search the plan space. 
Our work here focuses on the first component in our new domain of distributed protocols.

% \david{Cost models and automatic configuration.}
A natural next step is to develop cost models for our context, and integrate into a search algorithm.
% An automatic optimizer for distributed protocols can implement the rewrites introduced in this paper, given the ability to intelligently select an optimal configuration.
Standard techniques may be useful here, but we also expect new challenges in modeling dynamic load and contention, and focusing on bottleneck elimination. It seems likely that adaptive query optimization and learning could prove relevant here to enable autoscaling (\cite{deshpande2007adaptive,trummer2018skinnerdb}, etc.)

In addition to expanding this work with more functionality, it is also natural to apply this work to new challenges, including new protocols (e.g. BFT and blockchain), and  complex hardware environments. The latter is a topic of growing (manually-designed) interest in the distributed systems community~\cite{noPaxos, mu}.

Finally, because our work was inspired Whittaker, et al.'s manual rewrites~\cite{compartmentalized}, we inherited oversights of that work: it ensures safety, but makes no strong claims about liveness or failure handling. Correctly handling those concerns in our framework would improve the robustness of our optimized protocols.

% can provide such an optimizer with an estimate of the change in throughput when an optimization is applied; unlike query optimizers, these estimators must intelligently navigate the resulting change in load and contention as well.
% Automatic reconfiguration can allow protocols to adapt to changing workloads on-the-fly, allowing engineers to deploy protocols knowing it will scale to fit the workload.

% \nc{Don't need to devote as much time to natural extensions of this work (like BFT or hardware).
% Move discussion of safety and liveness here. We inherit the same limitations as Michael when handling failures and liveness, it's hard in general (cite Neils' hotstuff, ironfleet)}
% \david{BFT.}
% This paper assumes that all nodes are honest, so additional nodes can distribute the workload; in a byzantine setting, additional nodes might be malicious.
% Adapting this work to BFT would require a new definition of correctness and modifications to our existing optimizations.

% \david{Hardware.}
% The resurgence of specialized hardware has led to a suite of new distributed protocols~\cite{noPaxos,mu}.
% An automatic optimizer can identify subcomponents of programs that can run on specialized hardware and decouple them from the rest of the protocol.
